Probabilistic Counting in Generalized Turnstile Models

Traditionally in the turnstile model of data streams, there is a state vector $x=(x_1,x_2,\ldots,x_n)$ which is updated through a stream of pairs $(i,k)$ where $i\in [n]$ and $k\in \Z$. Upon receiving $(i,k)$, $x_i\gets x_i + k$. A distinct count algorithm in the turnstile model takes one pass of the stream and then estimates $\norm{x}_0 = |\{i\in[n]\mid x_i\neq 0\}|$ (aka $L_0$, the Hamming norm). In this paper, we define a finite-field version of the turnstile model. Let $F$ be any finite field. Then in the $F$-turnstile model, for each $i\in [n]$, $x_i\in F$; for each update $(i,k)$, $k\in F$. The update $x_i\gets x_i+k$ is then computed in the field $F$. A distinct count algorithm in the $F$-turnstile model takes one pass of the stream and estimates $\norm{x}_{0;F} = |\{i\in[n]\mid x_i\neq 0_F\}|$. We present a simple distinct count algorithm, called $F$-\pcsa{}, in the $F$-turnstile model for any finite field $F$. The new $F$-\pcsa{} algorithm takes $m\log(n)\log (|F|)$ bits of memory and estimates $\norm{x}_{0;F}$ with $O(\frac{1}{\sqrt{m}})$ relative error where the hidden constant depends on the order of the field. $F$-\pcsa{} is straightforward to implement and has several applications in the real world with different choices of $F$. Most notably, it makes distinct count with deletions as simple as distinct count without deletions.

==> text.tex <==

Other connections between sketching and algebra have been explicitly or implicitly established before in a range of streaming problems. To list a few,  $p$-stable random variables on $\R$ (which is typically not available in other spaces) are suitable to sketch $(0,2]$-frequency moments (\cite{cormode2003comparing}, \cite{indyk2006stable}); Roots of $x^k=1$ on the complex unit circle (which enjoy the algebraic properties of $\C$) are suitable to sketch $[2,\infty)$-frequency moments (\cite{alon1996space},\cite{ganguly2004estimating}) and the number of $d$-regular subgraphs in a dynamic graph (\cite{jowhari2005new},\cite{manjunath2011approximate}). 
